Crossing the Linguistic Causeway: Ethnonational Differences on Soundscape Attributes in Bahasa Melayu

Despite being neighbouring countries and sharing the language of Bahasa Melayu (ISO 639-3:ZSM), cultural and language education policy differences between Singapore and Malaysia led to differences in the translation of the "annoying" perceived affective quality (PAQ) attribute from English (ISO 639-3:ENG) to ZSM. This study expands upon the translation of the PAQ attributes from eng to ZSM in Stage 1 of the Soundscapes Attributes Translation Project (SATP) initiative, and presents the findings of Stage 2 listening tests that investigated ethnonational differences in the translated ZSM PAQ attributes and explored their circumplexity. A cross-cultural listening test was conducted with 100 ZSM speakers from Malaysia and Singapore using the common SATP protocol. The analysis revealed that Malaysian participants from non-native ethnicities (my:o) showed PAQ perceptions more similar to Singapore (sg) participants than native ethnic Malays (MY:M) in Malaysia. Differences between Singapore and Malaysian groups were primarily observed in stimuli related to water features, reflecting cultural and geographical variations. Besides variations in water source-dominant stimuli perception, disparities between MY:M and SG could be mainly attributed to vibrant scores. The findings also suggest that the adoption of region-specific translations, such as membingitkan in Singapore and menjengkelkan in Malaysia, adequately addressed differences in the annoying attribute, as significant differences were observed in one or fewer stimuli across ethnonational groups The circumplexity analysis indicated that the quasi-circumplex model better fit the data compared to the assumed equal angle quasi-circumplex model in ISO/TS 12913-3, although deviations were observed possibly due to respondents' unfamiliarity with the United Kingdom-centric context of the stimulus dataset...

==> table/modelfit.tex <==
\begin{table}
\footnotesize
\caption{\label{tab:modelfit}Summary of model fitting indexes and suggested threshold values that indicate a good fit}
\centering
\begin{tabularx}{\linewidth}{p{1.1cm}lllll}
\toprule
Indices
& CI ($p$) 
& SSM
& CFI 
& RMSEA 
& SRMR\\
\midrule
Thresholds
& $>0.7$
& $>0.7$
& $>0.92$
& $<0.08$
& $<0.08$\\
\midrule
MY:M & 0.597 (0.002) & 0.395 & 0.734 & 0.254 & 0.254\\
MY:O & 0.681 (0.002) & 0.637 & 0.825 & 0.185 & 0.217\\
SG & \textbf{0.701} (0.002) &\textbf{0.706} & 0.656 & 0.293 & 0.231\\
\bottomrule
\end{tabularx}
\end{table}


==> table/modelfitnew.tex <==
\begin{table}

\caption{\label{tab:modelfitnew}Summary of model fitting indexes, where conformity to the recommended threshold is indicated in \textbf{bold}}
\centering
\begin{tabularx}{\linewidth}{{>{\raggedright\arraybackslash}p{1.2cm}}X*{3}{>{\centering\arraybackslash}p{1.1cm}}}
\toprule
  &  & MY:M & MY:O & SG\\
\midrule
\multicolumn{5}{l}{\textit{Circular order}} \\
CI ($p$) &  & 0.597 (0.002) & 0.681 (0.002) & 0.701 (0.002)\\
\midrule
\multicolumn{5}{l}{\textit{Quasi-circumplex}} \\
CFI & $\ge0.90$ & \textbf{1.000} & \textbf{1.000} & \textbf{1.000}\\
RMSEA & $\le0.13$ & \textbf{0.000} & \textbf{0.000} & \textbf{0.000}\\
SRMSR & $<0.06$ & \textbf{0.016} & \textbf{0.020} & \textbf{0.037}\\
\midrule
\multicolumn{5}{l}{\textit{Equal angles}} \\
CFI & $\ge0.90$ & 0.734 & 0.825 & 0.656\\
RMSEA & $\le0.13$ & 0.254 & 0.185 & 0.293\\
SRMSR & $<0.06$ & 0.254 & 0.217 & 0.231\\
\midrule
\multicolumn{5}{l}{\textit{Equal communality}} \\
CFI & $\ge0.90$ & \textbf{0.992} & \textbf{0.907} & 0.881\\
RMSEA & $\le0.13$ & \textbf{0.044} & 0.134 & 0.172\\
SRMSR & $<0.06$ & 0.114 & 0.108 & 0.142\\
\midrule
\multicolumn{5}{l}{\textit{Equal communality and angles}} \\
CFI & $\ge0.90$ & 0.543 & 0.611 & 0.486\\
RMSEAe& $\le0.13$ & 0.282 & 0.234 & 0.305\\
SRMSR & $<0.06$ & 0.307 & 0.237 & 0.269\\
\midrule
\multicolumn{5}{l}{\textit{Circulant (Equal communality and angles)}} \\
SSM & $\ge 0.7$ & 0.395 & 0.637 & \textbf{0.706}\\
\bottomrule
\end{tabularx}
\end{table}


==> table/modelfitnew2.tex <==
\begin{table}

\caption{\label{tab:modelfitnew}Summary of model fitting indexes}
\centering
\begin{tabu}{llllll}
\toprule
  &  & MY:M & MY:O & SG & ARAUS\\
\midrule
CI (p) &  & 0.597 (0.002) & 0.681 (0.002) & 0.701 (0.002) & 0.847 (0)\\
CFIq & \textbackslash{}ge0.90 & 1.000 & 1.000 & 1.000 & 1.000\\
RMSEAq & \textbackslash{}ge0.13 & 0.000 & 0.000 & 0.000 & 0.000\\
SRMRq & < 0.06 & 0.016 & 0.020 & 0.037 & 0.023\\
CFIea & \textbackslash{}ge0.90 & 0.734 & 0.825 & 0.656 & 0.949\\
RMSEAea & \textbackslash{}ge0.13 & 0.254 & 0.185 & 0.293 & 0.097\\
SRMRea & < 0.06 & 0.254 & 0.217 & 0.231 & 0.159\\
CFIec & \textbackslash{}ge0.90 & 0.992 & 0.907 & 0.881 & 1.000\\
RMSEAec & \textbackslash{}ge0.13 & 0.044 & 0.134 & 0.172 & 0.000\\
SRMRec & < 0.06 & 0.114 & 0.108 & 0.142 & 0.056\\
CFIeca & \textbackslash{}ge0.90 & 0.543 & 0.611 & 0.486 & 0.965\\
RMSEAeca & \textbackslash{}ge0.13 & 0.282 & 0.234 & 0.305 & 0.068\\
SRMReca & < 0.06 & 0.307 & 0.237 & 0.269 & 0.168\\
SSM & > 0.7 & 0.395 & 0.637 & 0.706 & 0.803\\
\bottomrule
\end{tabu}
\end{table}

